Requirements Intelligence with OpenReq Analytics

With the rise of social media like Twitter and distribution platforms like app stores, users have various ways to express their opinions about software products. Popular software vendors get user feedback thousandfold per day. Research has shown that such feedback contains valuable information for software development teams. However, a manual analysis of user feedback is cumbersome and hard to manage. We present OpenReq Analytics, a software requirements intelligence service, that collects, processes, analyzes, and visualizes user feedback.

==> annex.tex <==
\section*{Annex}
\subsection{How the tool will be presented}
We will present \emph{OpenReq Analytics} in an interactive demonstration and a short introductory video.

\textbf{Interactive Demonstration.}
The tool can be reached under the following url: \url{http://analytics.openreq.eu}.
At the conference we will have a guided demonstration of the tool in its live environment.
During that demonstration, we will introduce the European HORIZON 2020 project OpenReq and its goals.
We further explain how and why we are developing the tool and in which industry scenarios it is currently tested and useful.

\textbf{Video.}
We will also show a video that explains how \emph{OpenReq Analytics} is used by our industry partners.
In that video the industry partners explain the problems---in terms of requirements engineering---they are facing, how \emph{OpenReq Analytics} helps them, and how their continuous feedback is shaping the tool.

\subsection{Further documentation}
Every component of the European HORIZON 2020 project OpenReq is open source, and so are all microservices of \emph{OpenReq Analytics}\footnote{\url{https://github.com/OpenReqEU}}.
Despite the code being publicly available, we also document all API endpoints of our components\footnote{\url{https://api.openreq.eu}}.
In our demonstration, we will stress both points as we want to encourage participation with interested researchers and practitioners also after the conference. 

\clearpage
\begin{figure*}[tb]
    \centering
    \includegraphics[width=\textwidth, height=12cm]{figure/dashboard.png}
    \caption{Requirements Intelligence - Dashboard}
\end{figure*}
\begin{figure*}[tb]
    \centering
    \includegraphics[width=\textwidth, height=8cm]{figure/focus_view.png}
    \caption{Requirements Intelligence - Focus View for Inquiries}
\end{figure*}
